Multiwavelength Observations of the Blazar PKS 0735+178 in Spatial and Temporal Coincidence with an Astrophysical Neutrino Candidate IceCube-211208A

We report on multiwavelength target-of-opportunity observations of the blazar PKS 0735+178, located 2.2$^\circ$ away from the best-fit position of the IceCube neutrino event IceCube-211208A detected on December 8, 2021. The source was in a high-flux state in the optical, ultraviolet, X-ray, and GeV gamma-ray bands around the time of the neutrino event, exhibiting daily variability in the soft X-ray flux. The X-ray data from Swift-XRT and NuSTAR characterize the transition between the low-energy and high-energy components of the broadband spectral energy distribution (SED), and the gamma-ray data from Fermi -LAT, VERITAS, and H.E.S.S. require a spectral cut-off near 100 GeV. Both X-ray and gamma-ray measurements provide strong constraints on the leptonic and hadronic models. We analytically explore a synchrotron self-Compton model, an external Compton model, and a lepto-hadronic model. Models that are entirely based on internal photon fields face serious difficulties in matching the observed SED. The existence of an external photon field in the source would instead explain the observed gamma-ray spectral cut-off in both leptonic and lepto-hadronic models and allow a proton jet power that marginally agrees with the Eddington limit in the lepto-hadronic model. We show a numerical lepto-hadronic model with external target photons that reproduces the observed SED and is reasonably consistent with the neutrino event despite requiring a high jet power.

==> martins_theory.tex <==
\subsection{Model Basics and SSC}
We shall firstly discuss the implications of an intrinsic gamma-ray cut-off at 100 GeV. The synchrotron spectrum peaks at a few $10^{14}$~Hz in frequency, or $\epsilon_\mathrm{max}=\epsilon_\mathrm{eV}$~eV in photon energy. \mpo{There will be a synchrotron-self-Compton contribution (SSC) to the SED.} If the Thomson limit applies, then the ratio between the \mpo{inverse-Compton (IC)} and the synchrotron peak frequencies gives the square of the maximum Lorentz factor of electrons, leading to 
\begin{equation}
\gamma_\mathrm{max}\simeq \frac{3\cdot 10^5}{\sqrt{\epsilon_\mathrm{eV}}}\ .
\end{equation}
The Thomson limit at $100$~GeV requires $\gamma \gg (2\cdot 10^5)/D=(8\cdot 10^3)/D_{25}$ which justifies a synchrotron peak up to the hard-UV band. The Swift XRT point at $300$~eV is already a factor of 30 below the UVOT points at $3$~eV, indicating that the cut-off energy is likely below $100$~eV, or $\epsilon_\mathrm{eV}\lesssim 100$. Close to this limit, the Klein-Nishina transition would add to the cut-off. 

\mpo{In the following any quantity measured in the jet frame is denoted with a prime (e.g. $R'$).} The synchrotron peak frequency constrains the magnetic-field strength \mpo{in the emission zone},
\begin{equation}
B' D\approx \frac{1.2\cdot 10^{-3}\ \mathrm{G}}{1+z}\,\epsilon_\mathrm{eV}^2\ ,
\label{eq:BD}
\end{equation}
where $D$ is the Doppler factor. We conclude that the magnetic field would have to be very weak.
At the same time, the jet-frame photon energy density at the synchrotron peak would have to be a factor of two or three larger than that in the magnetic field, \mpo{commensurate with the $\nu F_\nu$ flux ratio of the IC and the synchrotron peak.} We shall now see whether or not that is possible.

Assuming isotropic emission in the jet frame, at the distance \mpo{$d\approx 8.4\cdot 10^{27}\ \mathrm{cm}$, the intrinsic 
photon density per logarithmic energy interval and the energy density in the radiation field are
\begin{equation}
U'=\frac{3\,d^2}{c\,R'^2\,D^4}\, \nu F_\nu =\epsilon' n_\epsilon'
\label{eq:n_eps}
\end{equation}}
The $\nu F_\mu$ spectrum in the optical seems to be flat. Then the energy density of the synchrotron peak should be similar to that at $\epsilon\approx 1$~eV, corresponding to $\epsilon' \approx D^{-1}$~eV. We find \mpo{
\begin{equation}
U'\simeq
\frac{5\cdot 10^{-3}\ \mathrm{erg\,cm^{-3}}}
{D_{25}^4\,R_{16}^2}\, ,
\label{eq:u_eps}
\end{equation}}
where we denote the Doppler factor as $D=25\,D_{25}$ and the radius $R' = R_{16}\,(10^{16}\ \mathrm{cm})$.

The energy density in the magnetic field (cf. equation~\ref{eq:BD}) required for the SSC cut-off near 100 GeV and the synchrotron cut-off at $\epsilon_\mathrm{eV}$ is \mpo{
\begin{equation}
U_\mathrm{B}'\approx
(4\cdot 10^{-11}\ \mathrm{erg\,cm^{-3}})\,\frac{\epsilon_\mathrm{eV}^4}
{D_{25}^2}\ ,
\label{eq:u_B}
\end{equation}}
which is commensurate with the energy density of the photon field at the synchrotron peak only, if we pick a high synchrotron cut-off energy, $\epsilon_\mathrm{eV}\gtrsim 10$, and likely a large emission zone, $R_\mathrm{16}\gtrsim 10$. More precisely, we require that \mpo{
\begin{equation}
\epsilon_\mathrm{eV}\simeq \frac{100}{\sqrt{D_{25}\,R_{16}}}\ 
\label{eq:flux}.
\end{equation}}
The flux variation time scale should be at least as large as the electron cooling time, here about a third of the synchrotron cooling time, and be commensurate with daily flux variations (see Section~\ref{sec:res_var}). We find in the observer frame \mpo{
\begin{equation}
\tau\simeq \frac{1}{3}\,\tau_\mathrm{syn}
\approx
(0.7\ \mathrm{hours})\,D_{25}^{11/4}\,R_{16}^{7/4} \ ,
\end{equation}}
where in the last step we used eq.~\ref{eq:flux}. Evidently a large emission zone is not helpful for rapid energy losses. We should add that the seemingly flat $\nu F_\nu$ spectrum between the optical and the peak at $\epsilon_\mathrm{eV} $ likely requires an activity state that is at least as long as the loss time of electrons radiating in the optical, \mpo{which is about ten times larger than that at best-fitting peak frequency (cf. eq.~\ref{eq:flux}) but still shorter than a day}.
The causality argument requires $R_{16} \lesssim 7\,D_{25}$ \mpo{for daily variations} and would support a modest size of the emission zone. \mpo{Diffusive escape primarily affects the inverse-Compton component in a SSC model and is here sufficiently slow, even if the diffusion coefficient is a large multiple of the Bohm rate.}

\mpo{We conclude that for a synchrotron peak that extends far into the UV band, the SED and in particular cut-off near $100$~GeV can be reasonably well explained with a one-zone SSC model.}

%text regarding SSC modeling
Following \citet{Bottcher02}, two sets of parameters, listed in Table~\ref{tab:SSCmodel}, were used to generate the one-zone SSC models shown in Figure~\ref{fig:sed}. 

\begin{table*}
%\centering
   \caption{ Parameters used for the one-zone SSC models shown in Figure~\ref{fig:sed}.  \\
   {\footnotesize $\Gamma$ and $\theta$ are the bulk Lorentz factor and the viewing angle of the emitting region in the jet, respectively; $B$ is the strength of the magnetic field; $R$ is the radius of the emitting region; $L_\text{inj}$ is the injection luminosity of the electrons (and positrons); $\gamma_\text{brk}$ and $\gamma_\text{max}$ are the break (due to cooling) and the maximum Lorentz factor of the electrons, respectively; $p$ is the injection spectral indices of the electrons; $\eta_\text{esc}$ is the escape parameter defined as the ratio between the escape time of the electrons and the light crossing time $R/c$. }
   }
    \label{tab:SSCmodel}
\begin{tabular}{ccccc ccccc} \hline \hline
\centering
State & $\Gamma$ & $\theta$ & $B$ & $R$ & $L_\text{inj}$ &  $\gamma_\text{break}$ & $\gamma_\text{max}$ & $p$  & $\eta_\text{esc}$ \\
      &         & $^{\circ}$   &  $10^{-2}$ G & $10^{16} $ cm      & $10^{46}$ erg s$^{-1}$ &           &    & & \\ \hline
% below are v44 z=0.18 (R_17)
  high   & 30 & 1.91 & 9 & 3.8 & 6.0 & $1.2\times10^{4}$ & $5\times10^{5}$  & 3.4 & 200 \\
  low   & 30 & 1.91 & 6 & 4.0 & 4.0 & $1.2\times10^{4}$ & $5\times10^{5}$  & 3.4 & 140 \\ \hline
  %2009$^1$ & 30 & - & 0.25 & 4.0 & - & 10.25 & 12.0 & - & 3.0 & - \\ \hline
\end{tabular}\\
\end{table*}

%%%%%%%%%
\subsection{Flux Variability}
\label{subsec:vardis}
%%%%%%%%%

The soft X-ray flux (0.3 -- 10 keV) varied on timescales of $\sim1$ day by more than a factor of 2. However, the hard X-ray (3 -- 40 keV) flux varied much slower and stayed within the statistical uncertainty of the two \nustar{} measurements.   

Using the parameters in Table~\ref{tab:SSCmodel}, we can calculate the Lorentz factor of the electrons that produce the soft X-ray synchrotron emission $\gamma_\text{syn} \approx 5.4 \times 10^4 (B/1G)^{-1/2} [\delta/(1+z)]^{-1/2} (\nu_\text{syn}/10^{16}\text{Hz})^{1/2}$. The electron Lorentz factor ranges between $\sim1\times10^5$ and $\sim6\times10^5$ for the observed 0.3 keV and 10 keV photons, respectively. These electrons are of the highest energy in the injection spectrum covering up to the maximum Lorentz factor $\gamma_\text{max}$, at which the synchrotron cooling time is less than 2 hours in the observer frame. 

\textcolor{green}{(soft X-ray produced by the highest energy particles with faster cooling? Need to calculate SSC cooling time for hard X-ray)}

From causality, the size of the emitting region can be constrained using the fastest observed variability timescale ($\sim$1 day; see Section~\ref{sec:res_var}) and the Doppler factor used in the SSC model, $R\lesssim\text{c}t_\text{var} \delta /(1+z) \approx 5\times 10^{16} \;\text{cm}$. 

\subsection{Neutrino analysis} 
\mpo{Having established that a simple SSC model can explain the SED observed from 0735+178, we shall now explore the viability of associated neutrino emission that the SSC scenario alone can not account for. A significant number of accelerated ions or simply protons must also exist in the jet. Neutrino emission through the pp channel require a huge particle density in the jet and hence a tremendously large jet power \citep[e.g.][]{2000A&A...354..395P}. More likely appears neutrino production through p$\gamma$ interactions \citep{1995PhR...258..173G}. The implications in the case of PKS~0735+178 depend on the origin of the photon field with which the energetic protons would interact \citep{2022arXiv220405060S}.}
\subsubsection{Locally produced target photons}
If there were no absorption \mpo{by BLR photons, the low observed} flux at 350 GeV would strongly constrain the possibility of neutrino production, on account of moderate EBL absorption at this energy \mpo{(for the nominal redshift $z=0.45$)} as well as negligible internal absorption for any reasonable size of the emission zone. If \mpo{TXS0506+056 \citep{2019NatAs...3...88G} and published analysis strategies \citep{2017ApJ...849...67A}} can serve as an example, one 170-TeV neutrino within 180 days corresponds to a neutrino flux 
\begin{equation}
E F_\nu (E) \approx 4\cdot 10^{-12} \ \mathrm{erg\,cm^{-2}\,s^{-1}}
\label{nuflux}
\end{equation}
\mpo{The neutrino flux should not be significantly higher than that, otherwise the hard X-ray flux from secondary electrons in 0735+178 would exceed the observed level \citep{2019NatAs...3...88G}.}

Very roughly speaking, the pion cascade and p-$\gamma$ pair production provide a similar gamma-ray flux at 350 GeV \citep{2017ApJ...843..109G}. The VERITAS upper limits are about a factor five lower, meaning the expectation value for neutrinos is \mpo{0.03 per month}. In that case the association would likely be a chance event.

We shall again denote the Doppler factor as $D=25\,D_{25}$. The proton energy is about twenty times the energy of the emergent neutrino, assuming interaction through the $\Delta$ resonance \citep{2010ApJ...721..630H}. The proton Lorentz factor in the jet frame,
\begin{equation}
\gamma_p' \approx \frac{1+z}{D} \frac{20\, E_\nu}{m_p c^2}\approx 2\cdot 10^5 D_{25}^{-1} ,
\end{equation}
can be considered a soft upper limit, because protons of higher energy would produce more neutrinos at higher energy, where they are easier to detect. The typical energy of the target photons in p-$\gamma$ interactions is 
\begin{equation}
\epsilon_\mathrm{target}' \approx \frac{E_\mathrm{thresh}}{2\,\gamma_p'}
\simeq D_{25}\,(1\ \mathrm{keV}).
\label{eq:epsilon}
\end{equation}
For the observer that would be $25$~keV, \mpo{in the energy band covered by NUSTAR. Assuming the hard X rays are produced co-spatially with the neutrinos and isotropically in the jet frame, we can estimate the jet-frame photon density as a function of the radius of the emission zone, $R'$. In analogy to the derivation of equation~\ref{eq:u_eps}, but for the hard X-rays with flux $\nu F_\nu \approx 2\cdot 10^{-12}\ \mathrm{erg\,cm}^2\,\mathrm{s}^{-1}$, we find for the jet-frame photon density 
\begin{equation}
n_\epsilon'\approx \frac{2\cdot 10^5\ \mathrm{cm^{-3}}}{D_{25}^4\, R_{16}^2} .
\end{equation}}
The cross section of p-$\gamma$ interaction is $\sigma_{p\gamma} \simeq 5\cdot 10^{-28}\ \mathrm{cm^2}$. With the inelasticity $K=0.2$ \citep{2000CoPhC.124..290M} we find for the energy-loss time of the radiating protons
\begin{equation}
\tau_{p\gamma}'\approx\frac{1}{K\,c\,n_\epsilon'\,\sigma_{p\gamma}}
\simeq D_{25}^4\, R_{16}^2\ \left(1.7\cdot 10^{12}\ \mathrm{s}\right) .
\end{equation}
In the observer frame that would correspond to a few thousand years. \mpo{Protons will diffusively escape from the emission zone in a much shorter time, and hence p-$\gamma$ interactions are inefficient.} To reach any kind of reasonable output, we need a source radius $R_{16}\lesssim 1$. That would also be called for, if the emitter were located inside the BLR.

The most important unknown input \mpo{in an estimate of} the proton injection luminosity is the observed duration of the active state, $T_\mathrm{act}$. Building on eq.~\ref{nuflux} we find the neutrino luminosity that gives one neutrino as
\begin{equation}
L_\nu'\simeq 
D_{25}^{-4} \,\left(\frac{18\ \mathrm{days}}{T_\mathrm{act}}\right)\,\left(8\cdot 10^{40} \ \mathrm{erg/s}\right) .
\end{equation}
The \mpo{required} proton injection luminosity is at least a factor $\tau_{p\gamma}'/T_\mathrm{act}'$ larger than that, \mpo{
\begin{equation}
L_p'\gtrsim  \frac{R_{16}^2}{D_{25}}\,\left(\frac{18\ \mathrm{days}}{T_\mathrm{act}}\right)^2\,\left(3\cdot 10^{45} \ \mathrm{erg/s}\right) .
\end{equation}
In the AGN frame, the kinetic power of the jet is approximately a factor $D^2$ larger and would exceed the Eddington limit \citep{2014Natur.515..376G}}, unless the activity state is much longer than 18 days. \mpo{The same problem arises for TXS~0506+056. Given the high X-ray flux (which could largely be produced by secondary electrons) there is no real problem to reproduce the SED of 0735+178 with a lepto-hadronic scenario, if the power requirement could be reduced \citep[see also][]{2022arXiv220405060S}. Spine-sheath models \citep[e.g.][]{2015MNRAS.451.1502T} need less power, but imply a coherent bright sheath that is a few parsec long, otherwise the activity cannot extend over two weeks or more.}

\subsubsection{Target photons from the BLR}
\mpo{The featureless optical spectrum of 0735+178 suggests that it may be a BL Lac. It has been noted that also in BL Lacs the jet may pass through a region harboring a significant jet-external photon field \citep{2022ApJ...926...95F} that for simplicity we shall call a BLR. The BLR is an external source of photons, which which high-energy protons could produce neutrinos. The main issue in this scenario is that the emission zone cannot be comoving with the jet, otherwise it would leave the BLR within about a day of observed time. Corresponding leptonic models have been developed by \citet{2004ApJ...613..725S}.}

To estimate the photon density inside the BLR, we assume that the accretion disk produces 10\% of the \mpo{observed} UV flux, \mpo{about} 10\% of which are rescattered. For a BLR of radius $R_\mathrm{BLR}=2$~pc and monoenergetic photons of energy $\epsilon_\mathrm{BLR}\simeq 15$~eV, the AGN frame density of photons inside it is
\begin{equation}
n_\epsilon\approx  7\cdot 10^5\ \mathrm{cm^{-3}} 
\ .
\end{equation}
The pair-production opacity within the BLR would be \mpo{around unity} for photons of about 200~GeV \citep{2010ApJ...717L.118P}, consistent with a scenario in which the sharp drop of observed flux near 100~GeV is at least partially caused by absorption in the BLR.

In the jet frame the photon density would increase by the jet Lorentz factor, $\Gamma$, and the mean energy of BLR photons would be 
\begin{equation}
n_\epsilon' \approx \Gamma_{25}\,(2\cdot 10^7\ \mathrm{cm^{-3}})\qquad
\epsilon_\mathrm{BLR}'\approx \Gamma_{25}\,(500\ \mathrm{eV})\ ,
\end{equation}
which is reasonably close to that estimated in eq.~\ref{eq:epsilon}, in particular considering the moderate energy reconstruction of the neutrino with IceCube. 

The energy-loss time of the radiating protons would be
\begin{equation}
\tau_{p\gamma}'
\simeq \frac{1.7\cdot 10^{10}\ \mathrm{s}}{\Gamma_{25}} \ ,
\end{equation}
and the proton injection luminosity would be
\begin{equation}
L_p'\gtrsim  \left(\frac{18\ \mathrm{days}}{T_\mathrm{act}}\right)^2\,\frac{3\cdot 10^{43} \ \mathrm{erg/s}}{\Gamma_{25}\,D_{25}^5} .
\end{equation}
The jet luminosity is about a factor $D^2$ larger and in \mpo{marginal agreement with the Eddington luminosity \citep{2002AJ....123.2352X}.}

The emission zone radius is not constrained in such an external hadronic model and can be determined by the leptonic emission processes. \mpo{IC scattering of BLR photons would be strongly Klein-Nishina suppressed and not play a role both for the SED and as an energy-loss process.}

%%%%%%%%%
\subsection{External Compton Scattering}
\label{subsec:ec}
%%%%%%%%%

placeholder? \textcolor{red}{should we leave it out for a limited scope? }
